Non-Blocking Concurrent Imperative Programming with Session Types

Concurrent C0 is an imperative programming language in the C family with session-typed message-passing concurrency. The previously proposed semantics implements asynchronous (non-blocking) output; we extend it here with non-blocking input. A key idea is to postpone message reception as much as possible by interpreting receive commands as a request for a message. We implemented our ideas as a translation from a blocking intermediate language to a non-blocking language. Finally, we evaluated our techniques with several benchmark programs and show the results obtained. While the abstract measure of span always decreases (or remains unchanged), only a few of the examples reap a practical benefit.

==> eptcsdata.tex <==
\providecommand{\firstpage}{64}
\providecommand{\publicationstatus}{I. Cervesato and M. Fern\'andez (Eds): Fourth International Workshop\\ on Linearity 2016 (LINEARITY'16)\\
EPTCS 238, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.238.7}{10.4204/EPTCS.238.7}}
\pdfoutput=1

